Enhanced Wide-Angle Steering with Multi-Mode Multi-Port Aperture Antenna Arrays

A novel concept for wide-angle scanning is proposed based on multi-mode multi-port antennas. The theory of multi-mode multi-port antennas based on aperture radiators is developed and applied towards the design of an antenna array consisting of multi-mode aperture radiators. An advanced beamforming algorithm is developed and implemented, making use of the higher degrees of freedom available to multi-mode multi-port antennas. The manufactured antenna array is measured and compared to the expected performance. Wide-angle steering up to $\pm77^\circ$ from broadside with respect to a scan loss of $3\,\mathrm{dB}$ is achieved in both the horizontal and vertical plane with no visible grating lobe.

==> figures/currents/legend_currents.tex <==
\begin{tikzpicture}[rotate=0,every node/.style={font=\footnotesize}]
    \newcommand{\cbheight}{50mm}
    \node[inner sep=0, outer sep=0, rectangle, ultra thick, draw] (colorbar) {\includegraphics[width=3mm,height=\cbheight,angle=0]{figures/currents/matlab-colorbar.pdf}};
    \node[above,rotate=90] at (colorbar.west) {$\mathbf{M}_{s,\mathrm{norm}}$ in dB};
    \node[right] at ($(colorbar.south east) + (0,1*\cbheight)$) {$0$};
    \node[right] at ($(colorbar.south east) + (0,0.8*\cbheight)$) {$-4$};
    \node[right] at ($(colorbar.south east) + (0,0.6*\cbheight)$) {$-8$};
    \node[right] at ($(colorbar.south east) + (0,0.4*\cbheight)$) {$-12$};
    \node[right] at ($(colorbar.south east) + (0,0.2*\cbheight)$) {$-16$};
    \node[right] at ($(colorbar.south east) + (0,0.0*\cbheight)$) {$-20$};
    \draw[thick] ($(colorbar.south east) + (0,0.8*\cbheight)$) -- ++(-1.5mm,0mm);
    \draw[thick] ($(colorbar.south east) + (0,0.6*\cbheight)$) -- ++(-1.5mm,0mm);
    \draw[thick] ($(colorbar.south east) + (0,0.4*\cbheight)$) -- ++(-1.5mm,0mm);
    \draw[thick] ($(colorbar.south east) + (0,0.2*\cbheight)$) -- ++(-1.5mm,0mm);
\end{tikzpicture}

==> figures/farfields_array/legend_phi.tex <==
% \documentclass[]{standalone}
% \usepackage{tikz}
% \usetikzlibrary{intersections}
% \usetikzlibrary{calc, arrows.meta}
% \usepackage{xcolor}
% \usepackage{times}

% \begin{document}

\begin{tikzpicture}[every node/.style={font=\footnotesize}]
\newcommand{\figW}{8.6}
\newcommand{\figH}{1.4}

\newcommand{\xA}{0.2}
\newcommand{\lineW}{0.5}

\definecolor{colA}{RGB}{17, 113, 190}
\definecolor{colB}{RGB}{221, 84, 0}
\definecolor{colC}{RGB}{237, 177, 32}
\definecolor{colD}{RGB}{133, 22, 209}
\definecolor{colE}{RGB}{59, 170, 50}
\definecolor{colF}{RGB}{47, 190, 239}
\definecolor{colG}{RGB}{209, 4, 139}
\definecolor{colH}{RGB}{255, 214, 10}
\definecolor{colI}{RGB}{101, 130, 253}

\def\colorList{{"colA", "colB", "colC", "colD", "colE", "colF", "colG", "colH", "colI"}}

% Outer rectangle
\draw[thick] (0,0) rectangle (\figW,\figH);

    % \newcounter{counter} % No need to define the counter again, as legend_theta already defines it
    \setcounter{counter}{0} % Ensure counter is zeroed
    \foreach \x in{0,2,...,4} {
    \foreach \y in {1.1, 0.7, 0.3} {
        \stepcounter{counter}
        \pgfmathsetmacro{\currentCol}{\colorList[\the\value{counter}-1]}
        \pgfmathtruncatemacro {\currentAng}{(\the\value{counter}-1)*10+90}
        \draw[\currentCol, line width=1.5pt] (\xA+\x, \y) -- (\xA+\x+\lineW, \y) node[right,black] {$\varphi = \currentAng^\circ$};
    }
    }

    \draw[gray, line width=1.5pt] (\xA + 6, 1.1) -- (\xA+\lineW + 6, 1.1) node[right,black] {Measurement};
    \draw[gray, line width=1.5pt,dashed] (\xA + 6, 0.7) -- (\xA+\lineW + 6, 0.7) node[right,black] {Simulation};

    % \foreach \c [count=\i] in \colorList {
    %     \node[fill=\c, text=white, minimum size=1cm] at (\i*1.5, 0) {\c};
    % }

    
\end{tikzpicture}

% \end{document}
